Surface excitations in the modelling of electron transport for electron- beam-induced deposition experiments

The aim of the present overview article is to raise awareness of an essential aspect that is usually not accounted for in the modelling of electron transport for focused-electron-beam-induced deposition (FEBID) of nanostructures: surface excitations are on the one hand responsible for a sizeable fraction of the intensity in reflection-electron-energy-loss spectra for primary electron energies of up to a few keV and, on the other hand, they play a key role in the emission of secondary electrons from solids, regardless of the primary energy. In this overview work we present a general perspective of recent works on the subject of surface excitations and on low-energy electron transport, highlighting the most relevant aspects for the modelling of electron transport in FEBID simulations.

==> mycommands.tex <==
% =======================================================================  
% Command definitions.

\newcommand{\Aal}{A_{\alpha\ell\kappa}}
\newcommand{\Aalp}{A_{\alpha\ell\kappa'}}
\newcommand{\ab}{\textbf{a}}
\newcommand{\Ab}{\textbf{A}}
\newcommand{\Abf}{\widetilde{\textbf{A}}}
\newcommand{\absrrp}{ {|\rb-\rpb|}}
\newcommand{\bb}{\textbf{b}}
\newcommand{\Bb}{\textbf{B}}
\newcommand{\Bcal}{\mbox{\boldmath $\mathcal{B}$}}
\newcommand{\Bcalm}{\mathcal{B}}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\bracket}[2]{\langle#1|#2\rangle}
\newcommand{\Cb}{\textbf{C}}
\newcommand{\cb}{\textbf{c}}
\newcommand{\Cov}[2]{{\rm Cov}\left(#1,#2\right)}
\newcommand{\Cor}[2]{\rho\left(#1,#2\right)}
\newcommand{\curl}{\nabla\times}
\newcommand{\Dacal}{\mbox{\boldmath $\mathcal{D}_\text{a}$}}
\newcommand{\Db}{\textbf{D}}
\newcommand{\db}{\textbf{d}}
\newcommand{\Dbcal}{\mbox{\boldmath $\mathcal{D}_\text{b}$}}
\newcommand{\Dcal}{\mbox{\boldmath $\mathcal{D}$}}
\newcommand{\Dcalf}{\widetilde{\mbox{\boldmath $\mathcal{D}$}}}
\newcommand{\Dcalm}{\mathcal{D}}
\newcommand{\dd}{{\rm d}}
\newcommand{\ee}{{\rm e}}
\newcommand{\Eacal}{\mbox{\boldmath $\mathcal{E}_\text{a}$}}
\newcommand{\Ebcal}{\mbox{\boldmath $\mathcal{E}_\text{b}$}}
\newcommand{\Ecal}{\mbox{\boldmath $\mathcal{E}$}}
\newcommand{\Ecalm}{\mathcal{E}}
\newcommand{\Ecalf}{\widetilde{\mbox{\boldmath $\mathcal{E}$}}}
\newcommand{\EF}{E_\textrm{F}}
\newcommand{\Ex}[1]{\left\langle #1 \right\rangle}
\newcommand{\Etildealk}{\tilde{E}_{\alpha \ell \kappa}}
\newcommand{\ea}{\epsilon_\text{a}}
\newcommand{\eb}{\epsilon_\text{b}}
\newcommand{\ellmax}{\ell_\textrm{max}}
\newcommand{\eu}{\hat{\textrm{e}}}
\newcommand{\fact}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
\newcommand{\fb}{\textbf{f}}
\newcommand{\Fb}{\textbf{F}}
\newcommand{\Fbf}{{\widetilde{\textbf{F}}}}
\newcommand{\gb}{\textbf{g}}
\newcommand{\Gb}{\textbf{G}}
\newcommand{\hb}{\textbf{h}}
\newcommand{\Hb}{\textbf{H}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\ii}{{\rm i}}
\newcommand{\intab}{\int_a^b}
\newcommand{\intBZ}{{\int_{\Omega_\textrm{BZ}}}}
\newcommand{\intR}{{\int_{\Omega_\textrm{R}}}}
\newcommand{\intfourpi}{\int_{4\pi}}
\newcommand{\intinfinf}{\int_{-\infty}^{\infty}}
\newcommand{\intinfzero}{\int_{\infty}^{0}}
\newcommand{\intminfinf}{\int_{\infty}^{-\infty}}
\newcommand{\intminfzero}{\int_{-\infty}^{0}}
\newcommand{\intmonepone}{\int_{-1}^1}
\newcommand{\intNOmega}{{\int_{\tilde{N}\Omega}}}
\newcommand{\intOmega}{{\int_\Omega}}
\newcommand{\intpitwopi}{\int_\pi^{2\pi}}
\newcommand{\intqmqp}{\int_{q_-}^{q_+}}
\newcommand{\intRthree}{{\int_\Rthree}}
\newcommand{\intRthreezdown}{{\int_{\Rthree,z\leq0}}}
\newcommand{\intRthreezup}{{\int_{\Rthree,z\geq0}}}
\newcommand{\intRtwo}{{\int_\Rtwo}}
\newcommand{\intWS}{{\int_{\Omega_\textrm{WS}}}}
\newcommand{\intzerokpf}{{\int_{|\kb'|\leq k_F}}}
\newcommand{\intzerokpfs}{{\int_{|\kb'|\leq k_F^\sigma}}}
\newcommand{\intzeroinf}{\int_0^{\infty}}
\newcommand{\intzeropi}{\int_0^{\pi}}
\newcommand{\intzerotwopi}{\int_0^{2\pi}}
\newcommand{\Jb}{\textbf{J}}
\newcommand{\jb}{\textbf{j}}
\newcommand{\jbf}{{\widetilde{\textbf{j}}}}
\newcommand{\kappab}{\bm{\kappa}}
\newcommand{\kappabu}{\hat{\bm{\kappa}}}
\newcommand{\Kb}{\textbf{K}}
\newcommand{\Kbu}{\hat{\textbf{K}}}
\newcommand{\Kcal}{\mbox{\boldmath $\mathcal{K}$}}
\newcommand{\Kmax}{K_\textrm{max}}
\newcommand{\kb}{\textbf{k}}
\newcommand{\kbin}{\textbf{k}_\textrm{in}}
\newcommand{\kbout}{\textbf{k}_\textrm{out}}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\kF}{{k_\textrm{F}}}
\newcommand{\kFs}{{k_\textrm{F}^\sigma}}
\newcommand{\kpar}{\textbf{k}_{\parallel}}
\newcommand{\kparm}{k_{\parallel}}
\newcommand{\kparw}{(\kpar,\omega)}
\newcommand{\kparmw}{(\kparm,\omega)}
\newcommand{\ktilde}{\widetilde{\textbf{k}}}
\newcommand{\ktildem}{\widetilde{\text{k}}}
\newcommand{\ku}{\hat{\textbf{k}}}
\newcommand{\Ku}{\hat{\Kb}}
\newcommand{\kw}{(\textbf{k},\omega)}
\newcommand{\kmw}{(k,\omega)}
\newcommand{\lb}{\textbf{l}}
\newcommand{\Lcalm}{\mathcal{L}}
\newcommand{\Mb}{\textbf{M}}
\newcommand{\mb}{\textbf{m}}
\newcommand{\mn}{m_\textrm{n}}
\newcommand{\melem}[3]{\langle#1|#2|#3\rangle}
\newcommand{\Nb}{\textbf{N}}
\newcommand{\Ncalh}{\hat{\mathcal{N}}}
\newcommand{\nsk}{{n\sigma\mathbf{k}}}
\newcommand{\nunit}{\hat{\textbf{n}}}
\newcommand{\Omegab}{\mbox{\boldmath $\Omega$}}
\newcommand{\OmegaBZ}{\Omega_{\textrm{BZ}}}
\newcommand{\Omegacell}{\Omega_{\textrm{cell}}}
\newcommand{\OmegaR}{\Omega_{\textrm{R}}}
\newcommand{\OmegaWS}{\Omega_{\textrm{WS}}}
\newcommand{\Pb}{\textbf{P}}
\newcommand{\Pcall}{\mathcal{P}_{\alpha\ell\kappa}}
\newcommand{\Pcallp}{\mathcal{P}_{\alpha\ell\kappa'}}
\newcommand{\PEcall}{\mathcal{P}_{E\ell}}
\newcommand{\Pleg}{P_\ell}
\newcommand{\pb}{\textbf{p}}
\newcommand{\partialt}{{\frac{\partial}{\partial t}}}
\newcommand{\partialtt}{{\frac{\partial^2}{\partial t^2}}}
%\newcommand{\qedsymbol}{\rule{1ex}{1ex}}
%\newcommand{\qed}{\mbox{}\hfill\qedsymbol}
\newcommand{\qb}{\textbf{q}}
\newcommand{\Qb}{\textbf{Q}}
\newcommand{\Qcall}{\mathcal{Q}_{\alpha\ell\kappa}}
\newcommand{\Qcallp}{\mathcal{Q}_{\alpha\ell\kappa'}}
\newcommand{\qu}{\hat{\mathbf{q}}}
\newcommand{\qpar}{\textbf{q}_{\parallel}}
\newcommand{\qparm}{q_{\parallel}}
\newcommand{\qparw}{(\qpar,\omega)}
\newcommand{\qparwab}{(\qpar,\omega;\text{a},\text{b})}
\newcommand{\qparmw}{(\qparm,\omega)}
\newcommand{\qw}{(\textbf{q},\omega)}
\newcommand{\qwab}{(\qb,\omega;\text{a},\text{b})}
\newcommand{\rb}{\textbf{r}}
\newcommand{\Rcal}{\mbox{\boldmath $\mathcal{R}$}}
\newcommand{\Rmin}{R_\textrm{min}}
\newcommand{\rhoa}{\rho_\text{a}}
\newcommand{\rhob}{\rho_\text{b}}
\newcommand{\rhof}{\tilde{\rho}}
\newcommand{\rhos}{\rho_\textrm{s}}
\newcommand{\rpar}{\textbf{r}_{\parallel}}
\newcommand{\rpart}{(\textbf{r}_{\parallel},t)}
\newcommand{\rpb}{\textbf{r}'}
\newcommand{\rt}{(\textbf{r},t)}
\newcommand{\rpt}{(\rpb,t)}
\newcommand{\Rb}{\textbf{R}}
\newcommand{\RMT}{R_\alpha}
\newcommand{\Rtwo}{{\mathbbm{R}^2}}
\newcommand{\Rthree}{{\mathbbm{R}^3}}
\newcommand{\ru}{\hat{\textbf{r}}}
\newcommand{\ssb}{\textbf{s}} % \sb is some stacking command already.
\newcommand{\ssbu}{\hat{\ssb}} % \sb is some stacking command already.
\newcommand{\Sb}{\textbf{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\seitz}[2]{\{#1\,|\,\textbf{#2}\}}
\newcommand{\sigmaf}{{\widetilde{\sigma}}}
\newcommand{\sk}{{\sigma\mathbf{k}}}
\newcommand{\ssu}{\hat{\ssb}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Tcalh}{\hat{\Tcal}}
\newcommand{\ualk}{u_{\alpha\ell\kappa}}
\newcommand{\ualkp}{u_{\alpha\ell\kappa'}}
\newcommand{\ualpkp}{u_{\alpha\ell'\kappa'}}
\newcommand{\ub}{\textbf{u}}
\newcommand{\ubsl}{\textbf{u}_{sl}}
\newcommand{\ubdsl}{\dot{\ub}_{sl}}
\newcommand{\UC}{U_\textrm{C}}
\newcommand{\Ucalheps}{\hat{\mathcal{U}}_\epsilon}
\newcommand{\Ueff}{U_\textrm{eff}}
\newcommand{\Uen}{U_\textrm{en}}
\newcommand{\UH}{U_\textrm{H}}
\newcommand{\unitx}{\hat{\textbf{x}}}
\newcommand{\unity}{\hat{\textbf{y}}}
\newcommand{\unitz}{\hat{\textbf{z}}}
\newcommand{\Uxc}{U_\textrm{xc}}
\newcommand{\vb}{\textbf{v}}
\newcommand{\Var}[1]{{\rm Var}\left(#1\right)}
\newcommand{\Veff}{V_\textrm{eff}}
\newcommand{\Ven}{V_\textrm{en}}
\newcommand{\VH}{V_\textrm{H}}
\newcommand{\Vxc}{V_\textrm{xc}}
\newcommand{\vpar}{\textbf{v}_{\parallel}}
\newcommand{\vphi}{{\varphi}}
\newcommand{\vphif}{{\widetilde{\varphi}}}
\newcommand{\vu}{\hat{\textbf{v}}}
\newcommand{\wtil}{\widetilde{\omega}}
\newcommand{\xb}{\textbf{x}}
\newcommand{\xu}{\widehat{\textbf{x}}}
\newcommand{\yu}{\widehat{\textbf{y}}}
\newcommand{\zerob}{\mathbf{0}}
\newcommand{\zu}{\widehat{\textbf{z}}}

% =======================================================================  
% Theorems.

\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Property}
%\newtheorem{theorem}{Theorem}[section]    %theorem 2.0.1
\newtheorem{theorem}{Theorem}              %theorem 1
\newtheorem{corollary}{Corollary}
%\newtheorem{proof}{Proof}              %theorem 1

% =======================================================================  
% Lengths.

% Turn off indentation of the first line
%\setlength{\parint}{0mm}

